Inertial Bregman Proximal Gradient under Partial Smoothness

This work considers an Inertial version of Bregman Proximal Gradient algorithm (IBPG) for minimizing the sum of two single-valued functions in finite dimension. We suppose that one of the functions is proper, closed, and convex but non-necessarily smooth whilst the second is a smooth enough function but not necessarily convex. For the latter, we ask the smooth adaptable property (smad) with respect to some kernel or entropy which allows to remove the very popular global Lipschitz continuity requirement on the gradient of the smooth part. We consider the IBPG under the framework of the triangle scaling property (TSP) which is a geometrical property for which one can provably ensure acceleration for a certain subset of kernel/entropy functions in the convex setting. Based on this property, we provide global convergence guarantees when the entropy is strongly convex under the framework of the Kurdyka-\L{}ojasiewicz (KL) property. Turning to the local convergence properties, we show that when the nonsmooth part is partly smooth relative to a smooth submanifold, IBPG has a finite activity identification property before entering a local linear convergence regime for which we establish a sharp estimate of the convergence rate. We report numerical simulations to illustrate our theoretical results on low complexity regularized phase retrieval.

==> parts/S4_numexp.tex <==

\section{Numerical experiments}\label{sec:numexp}
In this section, we discuss some numerical experiments to illustrate our theoretical results.
\subsection{Application to quadratic inverse problem}
We apply our theoretical results to a quadratic inverse problem namely: phase retrieval. Our goal is to recover a desired signal $\avx\in\bbR^n$ from quadratic measurements. The  forward model can be written as 
\[y=|A\avx|^2,\]
where $y\in\bbR^m$ is the observation or measurements and $A:\bbR^n\rightarrow\bbR^m$ is a linear operator. We can reformulate this problem as an optimization problem in such form
\begin{equation}\label{eq:phase_retrieval}
    \min\limits_{x\in\bbR^n}\Psi(x)=F(x)+ G(x) \eqdef\frac{1}{4m}\normm{y-|Ax|^2}^2+\lambda R(x), \quad \lambda>0.
\end{equation}
Let us observe that $F$  is a  semi-algebraic data fidelity term and that $F\in C^2(\bbR^n)$ but is nonconvex due to the quadratic measurements. Besides, $\nabla F$ is not Lipschitz continuous. Therefore, we associate to $F$ the following Legendre function 
\begin{equation}\label{eq:entropy}
\psi(x)=\frac{1}{4}\normm{x}^4+\frac{1}{2}\normm{x}^2. 
\end{equation}
$\psi\in C^2(\bbR^n)$ is full domain and $1-$strongly convex function with a gradient that is Lipschitz over bounded subsets of $\bbR^n$ \cite[Proposition~2.6]{godeme_provable_2023}. It is quite simple to see that $F$ is smooth relative to $\psi$ \cite[Lemma~5.1]{bolte_first_2017}. $R$ is a regularizer that is partly smooth which guarantees that the recovered signal has the same prior structure as the original signal $\avx$. $\Argmin(\Psi)$ is a non-empty compact set when  $\Psi$ is coercive. Since  $G$ is bounded from below, $\Psi$ is coercive if $F$ is coercive and this happens to be true when the linear operator $A$ is injective. We deduce that  Assumptions~\ref{assump_A}-\ref{assump_B} are fullfilled. 

 
\subsection{Experiments setup}
Let us consider for the experimental setup that $A$ is a standard Gaussian matrix \ie each value of $A$ is drawn from the same mean-zero and standard Gaussian variable. We consider the problem~\eqref{eq:phase_retrieval} with the given entropy~\eqref{eq:entropy}. We solve this problem using the Bregman Proximal Gradient Algorithm~\ref{alg:BPGBT}. Indeed, in this random case, $F$ is $L=3+\delta-$smooth with respect to $\psi$ , ($\delta>0$, small enough) \cite[Lemma~B.5]{godeme_provable_2023}. Therefore for each numerical experiment, we run the BPG with the constant step-size $\gamma=\frac{0.99}{3+10^{-4}}$.
\begin{example}\textbf{(\onenorm).} For any  $x\in\bbR^n$, the \onenorm is given by 
$R(x)=\norm{x}{1}\eqdef\sum_{i=1}^n|x_i|,$ which is partly smooth at any $x$ relative to the manifold
\[\calM=T_x\eqdef\left\{u\in\bbR^n:\supp(u)\subset\supp(x)\right\},\quad\supp(x)\eqdef\{i:x_i\neq0\}.\] 
 The desired signal is assumed to be sparse \ie to have $s=12$ non-zeros entries for a vector of size $n=128$. We recover the signal from $m=0.5\times 12^(1.5)\times\log(128)$ measurements. We have that   $\lambda=10^{-8}$. Figure~\ref{fig: solving_l1} shows the results of the recovery. The left side of Figure~\ref{fig: solving_l1} displays the relative error of the iterates with respect to the number of iterations. On the right side, we display the support of the iterates with respect to the number of iterations. We can observe in the right figure that the Bregman Proximal Gradient identifies the correct manifold after 300 iterations and converges to the true vector. Besides, in red lines with have the practical error, and in blue dashed lines, we have the predicted error by  Theorem~\ref{localthm}. We can observe the linear convergence rate of the iterates.
\begin{figure}[htbp]
\centering
\includegraphics[trim={0cm 8cm 0 8cm},clip,width=0.7\linewidth]{numexp/error_l1.pdf}
 \caption{Phase retrieval with the $\ell_1-$norm regularizer.}
\label{fig: solving_l1}
\end{figure}
\end{example}
\begin{example}\textbf{(\onetwonorm).} Let us assume that the set  of index $\{1,\cdots,n\}$ is partitioned into non-overlapping blocks $\calB$ such that: $\bigcup\limits_{b\in\calB}=\{1,\cdots,n\}$. The \onetwonorm  of $x$ is given by $R(x)=\norm{x}{1,2}\eqdef\sum_{b\in\calB}\normm{x_b}$ with $x_b=(x_i)_{i\in b}\in\bbR^{|b|}$. This function is partly smooth at $x$ with respect to the following submanifold
\[\calM=T_x\eqdef\bBa{u\in\bbR^n:\supp_{\calB}(u)\subset\calS_{\calB},\quad \calS_{\calB}\eqdef\bigcup\{b:x_{b}\neq0\}}.\]
For this setup, we consider the true signal of size $n=128$ with $2$ non-zeros blocks of size 8.  We aim to recover this signal from $m=0.5\times(2\times 8)^2\times\log(128)$ quadratic measurements. We choose $\lambda=10^{-8}$.
\begin{figure}[htbp]
\centering
\includegraphics[trim={0cm 8cm 11cm 8.75cm},clip,width=0.35\linewidth]{numexp/error_l12.pdf}
 \caption{Phase retrieval with the $\ell_{1,2}-$norm regularizer.}
\label{fig: solving_l1}
\end{figure}
\end{example}

\begin{example}\textbf{(Total  variation).} Let us consider $R_0\in\PSF{\calK x}{\calM_0}$ where $\calK:\bbR^n\rightarrow\bbR^m$ is a linear operator.

If $\calK$ satisfies the transversality condition $\ran(\calK)+\calT(\calK x)=\bbR^m,\forall x\in\calM_0$) then $R\eqdef R_{0}\circ\calK$ is partly smooth with respect to $\calM=\{u\in\bbR^n: \calK u\in\calM_0\}$. The Total variation is polyhedral and partly smooth at $x$ relative to
\[\calM=T_{x}\eqdef\{u\in\bbR^n:\supp(\calK u)\subset\supp(\calK x)\}.\] 
\begin{itemize}
    \item The ``analysis prior'' formulation uses an objective function of the form:
    \begin{equation}\label{eq:tv_prior}
    \Psi(x)=\frac{1}{4m}\normm{y-|Ax|^2}^2+\lambda \norm{\calK x}{1}, \quad \lambda>0.
\end{equation}
    For the numerical experiments, we consider the anisotropic Total Variation or TV semi-norm. In this case  $R_0=\norm{\cdot}{1}$ and $\calK=\TVop$ is the finite difference approximation of the derivative. The desired signal is a random square having $s=12$ jumps with $n=128$ mainly the signal is piecewise constant. We recover the signal from $m=0.5\times s^2\times\log(n)$ measurements. Since the proximity operator
    of the TV semi-norm is not explicit, we used the Bregman Primal-dual Splitting \cite{silveti-falls_stochastic_2021} to solve the problem. On the left side, the dashed blue line is the true signal, and the red line is the recovered signal,  we can observe that the signal is recovered. On the right side, we displayed relative error with respect to the number of iterations. 
    \begin{figure}[htbp]
\centering
%[trim={left bottom right top},clip]
\includegraphics[trim={0cm 7cm 0cm 7cm},clip,width=.75\linewidth]{numexp/tv_recon.pdf}
 \caption{Phase retrieval with the TV semi-norm.}
\label{fig: solving_tv}
\end{figure}

    \item  The ``synthesis prior'' formulation of the phase retrieval problem under the Total variation regularizer, the objective function takes the form
\begin{equation}\label{eq:tv_synthesis}
    \Psi(v)=\frac{1}{4m}\normm{y-|A\calW v|^2}^2+\lambda \norm{v}{1}, \quad \lambda>0.
\end{equation}
In this case, the reconstructed signal is given by  $x=\calW v$ where $\calW$ is the inverse transform of the linear operator $\calK$ with $v$ the transform coefficients. When the linear operator is an orthogonal transform we have that $\calW=\transp{\calK}$ and therefore the analysis and synthesis formulations are equivalent. For 1D signals, the recovery with the TV semi-norm can be performed using a shift-invariant Wavelet dictionary \cite{steidl_equivalence_2004}. 

For the numerical experiments, let us consider the 1-D shift invariant Haar dictionary which is formed by  the set of scaled and dilated Haar filters
\[
\chi_i^{(j)}=\frac{1}{2^{(j+1)}}\left\{\begin{aligned} &+1, &\si\quad 0\leq i<2^{j},\\
&-1, &\si  -2^{j}\leq i<0,\\
 &0 & \odwz, \end{aligned}\right.
\]
Therefore the  corresponding dictionary is given by
$\adj{\calW}x=(\chi^{(j)}\ast x)_{0\leq j\leq J_{\max}}$, the indices $j$ correspond to the resolution and  is bounded by $J_{\max}<\log_2(n)$.

  \begin{figure}[htbp]
\centering
%[trim={left bottom right top},clip]
\includegraphics[trim={0cm 7cm 0cm 7cm},clip,width=.75\linewidth]{numexp/tv_wavelet.pdf}
 \caption{Phase retrieval with the synthesis prior formulation.}
\label{fig: solving_tv_syn}
\end{figure}
\end{itemize}
  \end{example}
















==> parts/S5_escape_property.tex <==
\section{Escape property}

In this section, we assume that the Bregman proximal gradient is initialized with a random point and we show that it converges to a point that is a ``good'' critical point: we coin this analysis as an escape property of the method. The core of this analysis is the stable manifold theorem. When the objective function is sufficiently smooth with a Lipschitz continuous gradient (see \cite{lee_first-order_2019}), first-order methods avoid strict saddle points. If the gradient of the objective is not Lipschitz continuous (see \cite{godeme_provable_2023}), mirror descent with an appropriate kernel also escapes the strict saddle point. For nonsmooth function (see \cite{davis_proximal_2022}), euclidean proximal methods also avoid active strict saddle points. The following theorem aims to extend this phenomenon to the Bregman Proximal gradient applied to a nonsmooth composite function with a non-Lipschitz continuous gradient of the smooth part. 

\begin{theorem}\label{thm: glbl_escp}\textbf{(BPG: Escape property)} 
Consider the minimization problem $(\calP)$ under Assumption A-B and let $\xpa\in\crit{\Psi}$. Let us assume that $G\in\PSF{\xpa,-\nabla F(\xpa)}{\calM_{\xpa}}$ and that  $G$ is $\varrho$-weakly convex relative to $\psi$. If $\gamma\in\left]0,\min\bPa{\frac{1}{L},\frac{1}{\varrho}}\right[$, then  for almost all initializers $\xo\in\calM_{\xpa}$ near $\xpa$ of the Bregman Proximal Gradient method, the following holds: 
 The limit of the sequence converges to $\crit{\Psi}\backslash\strisad{\Psi}$.
\end{theorem}

\begin{proof} 
Let $\xpa\in\crit{\Psi}$ and $B_{\xpa}$ be a neighborhood of $\xpa$, let us define 
$$ 
\calV_{\xpa}\eqdef\calM_{\xpa}\cap B_{\xpa}=\left\{x\in B_{\xpa}: M(x)=0\right\},
$$
where $M$ is the $C^2-$smooth  function describing the manifold locally around the critical point $\xpa$. Since $G$  is $\varrho-$weakly convex relative to $\psi$ and $\psi$ is strongly convex thus  the manifold $\calM_{\xpa}$ is uniquely determine. By imitating the proof of \cite[Lemma~4]{lee_first-order_2019} we have 
\begin{align*}
\Phi(x)&=\bPa{\nabla\psi+\gamma\partial G}^{*}\Ppa{\nabla\psi(x)-\gamma\nabla F(x)}=\bPa{\nabla_{\calM_{\xpa}}\psi+\gamma\nabla_{\calM_{\xpa}}G}^{-1}\proj{T_{\xpa}}\Ppa{\nabla\psi(x)-\gamma\nabla F(x)},
\end{align*}
where the conjugate is taken over the space $\calV_{\xpa}$.
Moreover, $\bPa{\nabla_{\calM_{\xpa}}\psi+\gamma\nabla_{\calM_{\xpa}}G}^{-1}$ is a local diffeomorphism. Indeed, 
\[D\bPa{\nabla_{\calM_{\xpa}}\psi+\gamma\nabla_{\calM_{\xpa}}G}^{-1}=\bPa{\nabla^2_{\calM_{\xpa}}\psi+\gamma\nabla^2_{\calM_{\xpa}}G}^{-1},\] and we combine the inverse function theorem  with the   fact that along the tangent space, $T_{\xpa}$, $\psi+\gamma G$ is strongly convex \ie,  
\begin{align*}
    \nabla^2_{\calM_{\xpa}}\psi+\gamma\nabla^2_{\calM_{\xpa}}G\slon (1-\gamma\varrho) \nabla^2_{\calM_{\xpa}}\psi\slon (1-\gamma\varrho)\sigma_{\psi}\Id_{T_{\xpa}}. 
\end{align*}
The $L$-smad property of $F$ with respect $\psi$ implies that $\proj{T_{\xpa}}\Ppa{\nabla\psi(x)-\gamma\nabla F(x)}$ is a diffeomorphism  and $\mathrm{det}\Ppa{D\proj{T_{\xpa}}\Ppa{\nabla\psi(x)-\gamma\nabla F(x)}}\neq0$ (see \cite[Lemma A.3]{godeme_provable_2023}). We deduce that $\Phi$ is a  diffeomorphism and that $\forall x, \mathrm{det} D(\Phi(x))\neq 0$. Proposition~\ref{pro:unstableprop} shows that if $\xpa\in\strisad{\Psi}$ then $\xpa$ is an unstable fixed point of $\Phi$ accroding to \cite[Definition~2.11]{davis_proximal_2022}. We wind up the proof by applying the Centre stable manifold theorem  \cite[Corollary 1]{lee_first-order_2019} in $\calV_{\xpa}$. 
\end{proof}

